Ensemble knowledge distillation of self-supervised speech models

Distilled self-supervised models have shown competitive performance and efficiency in recent years. However, there is a lack of experience in jointly distilling multiple self-supervised speech models. In our work, we performed Ensemble Knowledge Distillation (EKD) on various self-supervised speech models such as HuBERT, RobustHuBERT, and WavLM. We tried two different aggregation techniques, layerwise-average and layerwise-concatenation, to the representations of different teacher models and found that the former was more effective. On top of that, we proposed a multiple prediction head method for student models to predict different layer outputs of multiple teacher models simultaneously. The experimental results show that our method improves the performance of the distilled models on four downstream speech processing tasks, Phoneme Recognition, Speaker Identification, Emotion Recognition, and Automatic Speech Recognition in the hidden-set track of the SUPERB benchmark.

==> tabs/results2.tex <==
\begin{table*}[ht]
\setlength\tabcolsep{2.5pt}
%\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{cl|cc|cc|cc|cc|ccc|c}
\toprule
& & & & \multicolumn{2}{c|}{PR (PER ↓ )} & \multicolumn{2}{c|}{SID (Acc ↑ )} & \multicolumn{2}{c|}{ER (Acc ↑ )} & \multicolumn{3}{c|}{ASR (WER ↓ )} & \\
& & method & \# para. & clean  & chime   & clean  & chime  & clean & chime  & clean  & chime & chime-real & rank\\
\midrule
&\multicolumn{12}{l}{w/o pred.} \\
%(x) & HB \& RHB \& WL & -\\
\midrule
(a) & DT. HB (baseline)~\cite{chang2022distilhubert}   & -    & 23M    & 35.50  & 42.70  & 74.33  & 71.25 & 54.67 & 53.85 & 65.64  & 74.05  & 74.21 & 12  \\
(b) &DT. WL (baseline) & -    & 23M    & 32.00    & 38.83 & 76.5   & 72.75 & 54.95 & 54.67 & 61.76  & 68.41  & 69.16 & 9  \\
\midrule
(c) & DT. HB \& WL    & avg.    & 23M    & 33.14 & 40.67 & \textbf{\emph{77.83}} & \textbf{\emph{73.92}}  & \emph{55.22}  & 54.67 & 61.85  & 69.75  & 70.94 & 7  \\
(d) & DT. HB \& WL    & concat. & 23M    & 33.95 & 41.51 & 75.83  & 71.75 & 54.67 & \emph{54.95}  & 62.17  & 70.36  & 69.47 & 10  \\
(e) & DT. HB \& WL    & multi. pred.   & 23M    & 32.46 & 39.57 & 75.00 & 72.50  & \emph{57.69}  & \textbf{\emph{56.59}}  & \emph{60.81} & 69.10   & \emph{68.64} & 4 \\
\midrule
(f) & DT. RHB (baseline)~\cite{RobustDistilHuBERT}  & -  & 23M    & 32.95 & 38.18 & 74.67  & 71.25 & 53.85 & 51.10  & 62.55  & 68.32  & 69.15 & 11 \\
\midrule
(g) & DT. HB \& RHB &  multi. pred.   & 23M    & \emph{32.30}  & 39.50  & \emph{76.17} & \textbf{\emph{73.92}}  & \emph{56.87}  & \emph{56.04}  & \emph{60.94} & \emph{67.80}  & \emph{69.12} & 6  \\
(h) & DT. RHB \& WL  &  multi. pred.   & 23M    & \textbf{\emph{31.02}}  & \textbf{\emph{37.33}}  & 75.17  &   70.58    & \emph{56.59}  & \emph{53.30} & \emph{59.48} & \textbf{\emph{66.27}} & \textbf{\emph{65.21}} & 5\\
(i) & DT. HB \& RHB \& WL &  multi. pred.   & 23M    & \emph{31.14}  & \emph{38.06}  & 75.75  & 71.50 & \textbf{\emph{59.07}}  & \emph{56.32}  & \textbf{\emph{59.37}} & \emph{66.50}  & \emph{68.86} & 3 \\
\midrule
(y) & DT. HB \& DT. RHB \& DT. WL & - & 70M & 32.96	& 38.96 &	74.25 &	70.92 & 56.59 & 52.75 & 62.40 & 69.03 & 68.62& 8\\
\bottomrule
\toprule
 & \multicolumn{12}{l}{w/ pred.}\\
\midrule
(j) & DT. WL (Tr3) & - & 34M & 28.63 & 33.99 & 79.83 & 76.75 & 60.16 & 57.14 & 52.02  & 60.88 & 59.41 & 1\\
(k) & DT. HB \& RHB \& WL & \multicolumn{1}{c}{multi. pred.} & 34M    & 31.03 & 37.64 & 76.00  & 71.00 & 59.62  & 55.49 & 58.92  & 65.85  & 66.84 & 2\\
\bottomrule
\end{tabular}
\caption{Evaluation results on clean testing sets and testing sets with CHiME3 background noise. DT. is the abbreviation of Distil. In the ``method'' column, we specify whether the teacher representations are aggregated by average (avg.), aggregated by concatenation (concat.) or learned by multiple sets of prediction heads (multi. pred.). The baselines of each model trained with EKD are the individually distilled versions of the teacher models involved in the ensembling process. The values that outperform their corresponding baselines are italicized. The best performance values of models without prediction heads are marked bold. The rank of each model represents the overall performance on the clean set of the four downstream speech processing tasks.}
\label{tab:results}
\end{table*}
